Boosting Private Domain Understanding of Efficient MLLMs: A Tuning-free, Adaptive, Universal Prompt Optimization Framework

Efficient multimodal large language models (EMLLMs), in contrast to multimodal large language models (MLLMs), reduce model size and computational costs and are often deployed on resource-constrained devices. However, due to data privacy concerns, existing open-source EMLLMs rarely have access to private domain-specific data during the pre-training process, making them difficult to directly apply in device-specific domains, such as certain business scenarios. To address this weakness, this paper focuses on the efficient adaptation of EMLLMs to private domains, specifically in two areas: 1) how to reduce data requirements, and 2) how to avoid parameter fine-tuning. Specifically, we propose a tun\textbf{\underline{I}}ng-free, a\textbf{\underline{D}}aptiv\textbf{\underline{E}}, univers\textbf{\underline{AL}} \textbf{\underline{Prompt}} Optimization Framework, abbreviated as \textit{\textbf{\ourmethod{}}} which consists of two stages: 1) Predefined Prompt, based on the reinforcement searching strategy, generate a prompt optimization strategy tree to acquire optimization priors; 2) Prompt Reflection initializes the prompt based on optimization priors, followed by self-reflection to further search and refine the prompt. By doing so, \ourmethod{} elegantly generates the ``ideal prompts'' for processing private domain-specific data. Note that our method requires no parameter fine-tuning and only a small amount of data to quickly adapt to the data distribution of private data. Extensive experiments across multiple tasks demonstrate that our proposed \ourmethod{} significantly improves both efficiency and performance compared to baselines.

==> tab/steps.tex <==
% \begin{table}[t]
% \centering
% % \captionsetup{font={small,stretch=1}, labelfont={bf}}
% \caption{Comparison of performance and average iteration steps between OPRO and \ourmethod{} results on InternVL2-2B.}
% \resizebox{0.8\columnwidth}{!}{% adjust width
% \renewcommand{\arraystretch}{1.25}
%     \begin{tabular}{c|c|c|c}
%         % \Xhline{1.5pt}
%         \midrule[2pt]
%         \textbf{Method} & \textbf{MLLM} & \textbf{Average performance} & \textbf{Average Iteration Steps} \\
%         % \hline
%         \midrule[1.5pt]
%         \textbf{OPRO} & InternVL2-2B & 38.5 & \textasciitilde 50  \\
%         \hline
%         \textbf{\ourmethod{}} & InternVL2-2B & 56.3 & \textasciitilde 25 \\
%         % \Xhline{1.5pt}
%         \midrule[2pt]
%     \end{tabular}
%     }
%     \label{tab:tab4}
% \end{table}
\begin{table}[t]
\centering
\resizebox{0.9\columnwidth}{!}{% adjust width
\renewcommand{\arraystretch}{1.25}
    \begin{tabular}{l|c|c}
        % \Xhline{1.5pt}
        \midrule[2pt]
        \textbf{Method} & \textbf{ \makecell{Average \\Performance} } & \textbf{\makecell{Iteration \\Steps}} \\
        % \hline
        \midrule[1.5pt]
        \textbf{OPRO} & 38.5 & 50+-n  \\
        \hline
        \rowcolor{blue!5} \textbf{\ourmethod{}} & 56.3 & 25+-n \\
        % \Xhline{1.5pt}
        \midrule[2pt]
    \end{tabular}
    }
    \caption{Comparison of performance and average iteration steps between OPRO and \ourmethod{} on InternVL2-2B.}
    \vspace{-0.5cm}
    \label{tab:steps}
\end{table}
